Action Recognition using Transfer Learning and Majority Voting for CSGO

Presently online video games have become a progressively favorite source of recreation and Counter Strike: Global Offensive (CS: GO) is one of the top-listed online first-person shooting games. Numerous competitive games are arranged every year by Esports. Nonetheless, (i) No study has been conducted on video analysis and action recognition of CS: GO game-play which can play a substantial role in the gaming industry for prediction model (ii) No work has been done on the real-time application on the actions and results of a CS: GO match (iii) Game data of a match is usually available in the HLTV as a CSV formatted file however it does not have open access and HLTV tends to prevent users from taking data. This manuscript aims to develop a model for accurate prediction of 4 different actions and compare the performance among the five different transfer learning models with our self-developed deep neural network and identify the best-fitted model and also including major voting later on, which is qualified to provide real time prediction and the result of this model aids to the construction of the automated system of gathering and processing more data alongside solving the issue of collecting data from HLTV.

==> algorithm.tex <==
\begin{algorithm}[http]
\SetAlgoLined
\KwResult{Here will be the result }
 initialization\\
 os.makedirs(test.directory)\\
\For{$ data$ $in$ $test.dataset:$}{
video = data ['Video\textunderscore url'] \\
action = data ['action']\\
video\textunderscore name = data ['Video\textunderscore url']\\
freme\textunderscore rate  = video.getframeRate()\\
count = 0 \newline
 \While{video is open}{
 frame\textunderscore id = video.getframeid()\\
 frame = video.read()\\
  \If{frame\textunderscore id \% frame\textunderscore rate = 0 :}{
  file\textunderscore name = test\textunderscore directory + video\textunderscore name + frame\textunderscore id+ count + action+ ".jpg"\\
  cv2.imwrite (filename, frame)\\
  count + = 1\\
  }
  }
images = test\textunderscore directory.images\\
\For{$image$ $in$ $images :$}{

prediction\textunderscore list = np.array(image)\\
prediction\textunderscore list =  base\textunderscore model.predict(prediction\textunderscore list)\\
prediction\textunderscore list.reshape()\\
prediction.append(model.predict (prediction\textunderscore list)\\

}
   
   most\textunderscore predicted = prediction.value\textunderscore count.max\textunderscore value()\\
predicted.append(y\textunderscore train.columns.values [most predicted])\\
test\textunderscore directory.clean()\\
prediction.clean()\\
}

 \caption{Test prediction algorithms}
\end{algorithm}


==> algorithm_2.tex <==
\begin{algorithm}[H]
\SetAlgoLined
\KwResult{Here will be the result }
 initialization\\
 \If{not directory}
 {
 os.makedirs(test.directory)\\
 }
\For{$ data$ $in$ $test.dataset:$}{
video = videoCapture(data['video'])\\
action =  data ['action']\\
video\textunderscore name = data ['video']\\
frame\textunderscore rate= video.getframeRate()\\
count = 0 \\
 \While{video is open}{

frame = video.read()\\
frame id = video.getframeid()\\
 \If{frame\textunderscore id \% frame\textunderscore rate = 0 :}{
 file\textunderscore name = test\textunderscore directory + video\textunderscore name + frame\textunderscore id+ count + action+ 'jpg \\
cv2.imwrite (filename, frame)\\
count + = 1\\
   
   }
   }
   }
 \caption{Video to frame conversion}
\end{algorithm}
